Target set selection with maximum activation time

A target set selection model is a graph $G$ with a threshold function $\tau:V\to \mathbb{N}$ upper-bounded by the vertex degree. For a given model, a set $S_0\subseteq V(G)$ is a target set if $V(G)$ can be partitioned into non-empty subsets $S_0,S_1,\dotsc,S_t$ such that, for $i \in \{1, \ldots, t\}$, $S_i$ contains exactly every vertex $v$ having at least $\tau(v)$ neighbors in $S_0\cup\dots\cup S_{i-1}$. We say that $t$ is the activation time $t_{\tau}(S_0)$ of the target set $S_0$. The problem of, given such a model, finding a target set of minimum size has been extensively studied in the literature. In this article, we investigate its variant, which we call TSS-time, in which the goal is to find a target set $S_0$ that maximizes $t_{\tau}(S_0)$. That is, given a graph $G$, a threshold function $\tau$ in $G$, and an integer $k$, the objective of the TSS-time problem is to decide whether $G$ contains a target set $S_0$ such that $t_{\tau}(S_0)\geq k$. Let $\tau^* = \max_{v \in V(G)} \tau(v)$. Our main result is the following dichotomy about the complexity of TSS-time when $G$ belongs to a minor-closed graph class ${\cal C}$: if ${\cal C}$ has bounded local treewidth, the problem is FPT parameterized by $k$ and $\tau^{\star}$; otherwise, it is NP-complete even for fixed $k=4$ and $\tau^{\star}=2$. We also prove that, with $\tau^*=2$, the problem is NP-hard in bipartite graphs for fixed $k=5$, and from previous results we observe that TSS-time is NP-hard in planar graphs and W[1]-hard parameterized by treewidth. Finally, we present a linear-time algorithm to find a target set $S_0$ in a given tree maximizing $t_{\tau}(S_0)$.

==> FPT-Alg-simplified.tex <==
\section{TSS-time is FPT in graphs of bounded local treewidth}\label{sec:FPT-Alg}
%\ig{This section is new}



In this section we provide an \FPT algorithm to solve the \textsc{GTSS-time} problem in graphs of bounded local treewidth (\cref{thm:FPT}). This result together the \NP-completeness result of \cref{thm:hard-apex} will yield the complexity dichotomy proved in \cref{thm:dichotomy}.
We first need to introduce some notation.
 %and another version of the \textsc{TSS-time} problem.

Let $G$ be a graph and $\tau$ be a \b{generalized} threshold function in $G$. Recall that {$\tau^*= \max_{v \in V(G)}\tau(v)$}. \b{We define $V_{\sf f} := \{ v \in V(G) \mid \tau(v) > d(v)\}$. Note that any target set for the target selection model $(G,\tau)$ needs to contain the whole set $V_{\sf f}$ of ``forced'' vertices.}

%of \emph{forced} vertices, we denote by $t_{\tau}(G,V_{\sf f})$ the maximum activation time $t_{\tau}(S_0)$ among all target sets $S_0$ of $G$ such that~$V_{\sf f} \subseteq S_0$.
%Clearly, $t_{\tau}(G,\emptyset) = t_{\tau}(G)$, hence deciding whether $t_{\tau}(G,V_{\sf f}) \geq k$, for a positive integer $k$, is equivalent to \pname{GTSS-time} if we consider threshold of any vertex in $V_{\sf f}$ greater than the degree while the threshold of any other vertex is maintained.

In the next lemma, we show that deciding whether there exists a target set with activation time {\sl at least} $k$ is equivalent to the {\sl exact} version.

\begin{lemma}\label{lem:equal-at-least}
For every graph $G$, every generalized threshold function $\tau$ in $G$, and every positive integer $k$, $t_{\tau}(G) \geq k$ if and only if there is target set $S_0 \subseteq V(G)$  such that  $t_{\tau}(S_0) = k$. 
%In particular, $t_{\tau}(G) \geq k$ if and only if there is target set $S_0 \subseteq V(G)$ such that  $t_{\tau}(S_0) = k$.
\end{lemma}

\begin{proof}
If there is target set $S_0 \subseteq V(G)$  such that  $t_{\tau}(S_0) = k$, then by definition $t_{\tau}(G) \geq k$, so let us focus on the forward direction. Let $S_0$ be a target set of $G$  such that $t_{\tau}(S_0) \geq k$, and let $S_0, S_1, S_2, \ldots, S_t$ be the partition of  $V(G)$ given by  $S_0$, where $t \geq k$. If $t=k$, then we are done. Otherwise, let $S_0' = S_0 \cup S_1 \cup \dots \cup S_{t-k}$. It can be easily verified that $S_0'$ is a target set of $G$ such that~$t_{\tau}(S_0') =~k$.
\end{proof}

%Let $G$ be a graph, let $v \in V(G)$, and let $p$ be a positive integer. By \emph{attaching $p$ triangles to $v$} we mean the operation of adding $p$ vertex-disjoint triangles to $G$ and identifying one vertex of each triangle with $v$. We call these triangles \emph{pendent triangles}.

We now define auxiliary graphs that will be used in the \FPT algorithm of \cref{thm:FPT}. The crucial property of these auxiliary graphs is that they have diameter $\Ocal(k)$, which will be exploited in order to bound their treewidth.  Let $G$ be a graph, let $\tau$ be a generalized threshold function in $G$, let $v \in V(G)$, and let $k$ be a positive integer. We define the pair $(G_{k}^v, \tau_k^v)$ such that~$G_{k}^v$ is a graph and $\tau_k^v$ is a generalized threshold function in $G_{k}^v$, as follows. Let $G_{k}^v = G[N_k[v]]$, that is, the subgraph of $G$ induced by the vertices at distance at most $k$ from $v$ in $G$, and let
%(that is, the induced subgraph of $G$ containing all vertices within distance at most $k$ from $v$)
%by attaching $\tau(u)$ triangles to every vertex $u$ that is at distance exactly $k$ from $v$ in $G$. We define $\tau_k^v:V(G_{k}^v)\to\NN$ so that
$\tau_k^v$ be defined such that, if $u \in N_{k-1}[v]$ then $\tau_k^v(u) = \tau(u)$, and  \b{$\tau_k^v(u) = d(u) +1$} otherwise. That is, the set of vertices at distance exactly $k$ from $v$ in $G$ belongs to the set $V_{\sf f}$ of forced vertices for the pair $(G_{k}^v, \tau_k^v)$, and this will be used in the proof of the next lemma, 
%Since every vertex at distance exactly $k$ from $v$ in $G$ has some neighbor in $N_{k-1}[v]$, it can be easily verified that $\tau_k^v$ is indeed a threshold function in $G_{k}^v$, and this is the only reason for which we have set $\tau_k^v(u) = 1$ for every vertex $u$ at distance exactly $k$ from $v$ in $G$. Nevertheless, the value of $\tau_k^v$ for those vertices will be irrelevant since, as stated in the next lemma, we will always include them in the set $V_{\sf f}$ of forced vertices that must belong to any target set. 
where we show that dealing with the auxiliary graphs $G_{k}^v$ is enough in order to solve the \textsc{GTSS-time} problem. \ig{Note that $(\tau_k^v)^* \leq \tau^* + 1$}

\begin{lemma}\label{lem:balls}
For every graph $G$, every generalized threshold function $\tau$ in $G$, and every positive integer~$k$, $t_{\tau}(G) \geq k$ if and only if there exists a vertex $v \in V(G)$ such that $t_{\tau_k^v}(G_{k}^v) \geq k$. %where $V_{\sf f}$ is the set of vertices at distance exactly $k$ from $v$ in~$G$.
\end{lemma}
\begin{proof} Suppose first that $t_{\tau}(G) \geq k$. By \cref{lem:equal-at-least}, there is target set $S_0 \subseteq V(G)$ such that~$t_{\tau}(S_0) = k$. Let $V(G) = S_0 \uplus S_1 \uplus \dots \uplus S_k$ be the partition of $V(G)$ into $k$ non-empty sets given by $S_0$,  and let $v$ be any vertex in $S_k$, and let $D_k^v$ be  the set of vertices at distance exactly~$k$ from $v$ in~$G$.  We claim that $t_{\tau_k^v}(G_{k}^v) \geq k$. Let $S_0^v = (S_0 \cap N_{k-1}(v)) \cup D_k^v$. We have to verify that $S_0^v$ is a target set of $G_{k}^v$ with $t_{\tau_k^v}(S_0^v) \geq k$. Since $S_0$ activates vertex $v$ at time exactly $k$ in $G$, $S_0 \cup \{u\}$ also activates vertex $v$ at time exactly $k$ for any vertex $u \in D_k^v$. Iterating this argument, it follows that $S_0 \cup D_k^v$ activates vertex $v$ at time exactly $k$ in $G$. Thus, $S_0^v$ activates vertex $v$ at time exactly $k$ in~$G_{k}^v$. As for the other vertices of $G_{k}^v$, since $S_0$ is a target set of $G$ and $D_k^v \subseteq S_0^v$, it follows that $S_0^v$ is indeed a target set of $G_{k}^v$  that activates $v$ at time exactly $k$, and therefore $t_{\tau_k^v}(G_{k}^v) \geq k$.

Conversely, suppose that there exists $v \in V(G)$ such that $t_{\tau_k^v}(G_{k}^v) \geq k$. Let $S_0^v$ be a target set of $G_{k}^v$ such that $t_{\tau_k^v}(S_0^v) \geq k$. Let $S_0 = S_0^v \cup (V(G) \setminus N_{k}[v])$. That is, $S_0$ contains $S_0^v$ and all vertices at distance at least $k+1$ from $v$ in $G$. Since necessarily $D_k^v \subseteq S_0^v$, $S_0$ also contains all vertices at distance exactly $k$ from $v$ in $G$. We claim that $S_0$ is a target set of $G$ with $t_{\tau}(S_0) \geq k$. The fact that~$S_0$ is a target set of $G$ follows from the hypothesis that $S_0^v$ is a target set of $G_{k}^v$ and the fact that $S_0$ contains all vertices at distance at least $k$ from $v$ in $G$. On the other hand, since~$t_{\tau_k^v}(S_0^v) \geq k$, $S_0^v \subseteq S_0$, and no vertex in $V(G) \setminus N_{k}[v]$ has a neighbor in the set~$N_{k-1}[v]$, it follows that $t_{\tau}(S_0) \geq k$, and therefore $t_{\tau}(G) \geq k$.
\end{proof}

The last ingredient that we need before proving \cref{thm:FPT} is to show that deciding whether $t_{\tau}(G) \geq k$ can be expressed by an \MSOone formula of appropriate length. 

%Note that, in particular, this applies to deciding whether $t_{\tau}(G,\emptyset) = t_{\tau}(G)\geq k$, that is, to the \textsc{TSS-time} problem.

\begin{lemma}\label{lem:MSOL}
 Given a graph $G$, a generalized threshold function $\tau$ in $G$, and a positive integer $k$, the problem of deciding whether $t_{\tau}(G) \geq k$ can be expressed by an~\MSOone formula $\phi$ whose length depends on $k$ and $\tau^*$.
%The \textsc{TSS-time} problem, with instances of the form $(G, \tau, k)$, can be expressed by an \MSOone formula $\phi$ whose length depends on $k$ and $\max_{v \in V(G)}\tau(v)$.
\end{lemma}
\begin{proof}
We may assume that $G$ is given along with a partition of $V(G)$ according to the values of the threshold function $\tau$, namely $V(G) = V_0 \uplus V_1 \uplus \dots \cup V_{\tau^{\star}}$, where~$\tau^{\star} = \max_{v \in V(G)}\tau(v)$ and, for $j \in [0,\tau^{\star}]$, $V_j = \{v \in V(G) \mid \tau(v) = j\}$. Note that $V_{\sf f}$ and the sets $V_j$ may be empty. By \cref{lem:equal-at-least}, $(G, \tau, k)$ is a \yes-instance of \textsc{TSS-time} if and only there exists a target set $S_0 \subseteq V(G)$ such that $t_{\tau}(S_0) = k$. The existence of such a set~$S_0$ can be equivalently expressed as the existence of
 a partition $V(G)= S_0 \uplus S_1 \uplus \dots \uplus S_k$ into~$k+1$ non-empty sets such that \ig{HERE}
 \begin{enumerate}
\item[(i)] for every $i \in [2,k]$ and every $j \in  [0,\tau^{\star}]$, every vertex in $S_i \cap V_j$ has strictly less than $j$ neighbors in the set $\bigcup_{h=0}^{i-2}S_h$, and
\item[(ii)] for every $i \in [1,k]$ and every $j \in  [0,\tau^{\star}]$, every vertex in $S_i \cap V_j$ has at least $j$ neighbors in the set $\bigcup_{h=0 }^{i-1}S_h$.
\end{enumerate}
Let us argue that the above conditions can be indeed expressed by an \MSOone formula $\phi$ whose length depends only on $k$ and $\tau^*$. First, note that the existence of $k+1$ pairwise disjoint vertex sets that form a partition of $V(G)$ with $V_{\sf f} \subseteq S_0$ can be easily expressed in~\MSOone. On the other hand, in order to express condition~(i) above, it suffices to quantify, for every~$i \in [2,k]$, every $j \in  [0,\tau^{\star}]$, and every vertex $v \in S_i \cap V_j$, the non-existence of $j$ neighbors of $v$ in the set $\bigcup_{h=0}^{i-2}S_h$. Finally, as for condition~(ii), it suffices to quantify, for every $i \in [1,k]$, every $j \in  [0,\tau^{\star}]$, and every vertex $v \in S_i \cap V_j$, the existence of $j$ neighbors of~$v$ in the set $\bigcup_{h=0}^{i-1}S_h$. Clearly, the length of the obtained \MSOone formula $\phi$ is bounded by a function of $k$ and $\tau^*$, and the lemma follows.
\end{proof}

%\ig{Note that \cref{thm:NPC} proves that the \textsc{TSS-time} problem is \NP-complete even for fixed $k=4$ and $ \tau^{*} = 2$}
We finally have all the ingredients to prove our \FPT algorithm to solve the \textsc{TSS-time} problem. For a graph class ${\cal C}$, we denote by \textsc{TSS-time}$|_{{\cal C}}$ the restriction of the \textsc{TSS-time} problem to input graphs $G$ belonging to ${\cal C}$.

\begin{theorem}\label{thm:FPT}
If ${\cal C}$ is a graph class of bounded local treewidth, then the \textsc{TSS-time}$|_{{\cal C}}$ problem is \FPT parameterized by $k$ and $\tau^*$.
\end{theorem}
\begin{proof} Let $(G, \tau, k)$ be an instance of \textsc{TSS-time} where $G \in {\cal C}$, $\tau$ is a threshold function in $G$ and $k$ is a positive integer. Since ${\cal C}$ has bounded local treewidth, there exists a function~$f:\NN \to\NN$  such that, for every graph $G\in{\cal C}$, every vertex $v \in V(G)$ and every positive integer $r$, $\tw(G[N_r[v]])\leq f(r)$.

By \cref{lem:balls}, $t_{\tau}(G) \geq k$ if and only if there exists a vertex $v \in V(G)$ such that~$t_{\tau_k^v}(G_{k}^v, V_{\sf f}) \geq k$, where $V_{\sf f}$ is the set of vertices at distance exactly $k$ from $v$ in~$G$. Based on this, for every vertex $v \in V(G)$, we generate in linear time the graph $G_{k}^v$, and it is enough to decide whether $t_{\tau_k^v}(G_{k}^v, V_{\sf f}) \geq k$. Since $G_{k}^v = G[N_k[v]]$ and $G \in {\cal C}$, we have that~$\tw(G_{k}^v) \leq f(k)$.
By \cref{lem:MSOL}, deciding whether $t_{\tau_k^v}(G_{k}^v, V_{\sf f}) \geq k$ can be expressed by an \MSOone (in particular, \MSO) formula $\phi$ whose length depends only on $k$ and~$\tau^*$. Therefore,
 \cref{thm:Courcelle} implies that deciding whether $t_{\tau_k^v}(G_{k}^v, V_{\sf f}) \geq k$ can be solved in time~$g(k, \tau^*, \tw(G_{k}^v)) \cdot n$ for some computable function $g$, where $n = |V(G)|$. Since
$\tw(G_{k}^v) \leq f(k)$, deciding whether~$t_{\tau}(G) \geq k$ can be solved in time~$h(k, \tau^*) \cdot n^2$ for some computable function~$h:\Bbb{N}^{2}\to\Bbb{N}$, and the theorem follows.
\end{proof}

As particular cases of \cref{thm:FPT}, it follows that the \textsc{TSS-time}$|_{{\cal C}}$ problem is \FPT parameterized by $k$ and $\tau^*$ when ${\cal C}$ is the class of graphs of treewidth bounded by a constant, the class of graphs of maximum degree bounded by a constant, the class of planar graphs or, more generally, the class of graphs embeddable in a fixed surface (i.e., bounded genus graphs).

%\begin{corollary}\label{cor:FPT}
%Diameter-treewidth property, planar, bounded genus, bounded treewidth...
%\qed\end{corollary}

With \cref{thm:hard-apex} and \cref{thm:FPT} at hand, the following dichotomy theorem can be easily proved.

\begin{theorem}\label{thm:dichotomy}
Let ${\cal C}$ be a minor-closed graph class.  Then  \textsc{TSS-time}$|_{{\cal C}}$ is% \vspace{-.25cm}
\begin{itemize}
\item[$\bullet$] \FPT parameterized by $k$ and $\tau^*$, if ${\cal C}$ has bounded local treewidth.
\item[$\bullet$] \NP-complete for every fixed $k \geq 4$ and $ \tau^{*} = 2$, otherwise.
\end{itemize}
\end{theorem}
\begin{proof}
Let ${\cal C}$ be a minor-closed graph class. If ${\cal C}$ has bounded local treewidth, the result follows from \cref{thm:FPT}.  Otherwise, \cref{thm:Eppstein} implies that ${\cal C}$ contains all apex graphs, and by \cref{thm:hard-apex} the \textsc{TSS-time}$|_{{\cal C}}$ problem is  \NP-complete for every fixed $k \geq 4$ and $ \tau^{*} = 2$.
\end{proof} 

==> PolyTrees-General.tex <==
\section{\pname{generalized TSS-time} is polynomial in trees}
\label{sec:PolyTreesG}

%In this section, we generalize the result for trees presented in \cref{sec:PolyTrees} by allowing thresholds equal to 0. We also generalize the result to pairs $(G,\tau)$ that are not instances of \c{TSS} \igr{\textsc{TSS-time}}: $\tau(v)>d(v)$ is possible (\b{we stress that this is allowed} only in this section). The main difference is that every target set $S_0$ must contain each vertex $v$ with $\tau(v)>d(v)$, since such a vertex $v$ cannot be activated by its neighbors. Moreover, in the computation of the maximum activation time, we may assume that any target set $S_0$ does not contain any vertex $v$ with $\tau(v)=0$, since such a vertex will always be activated at time 1.

Given a graph $G$, a vertex subset $S_0\subseteq V(G)$, and a vertex $v$ of $G$, recall that $t_{\tau}(v,S_0)$ is the minimum integer $k$ such that $v\in I^k(S_0)$, or $t_{\tau}(v,S_0)=\infty$ if $v\not\in H(S_0)$. By applying the algorithm \pname{Activation-Times} over a set $S_0$, we have that $H(S_0)$ and $t_{\tau}(v,S_0)$ for every vertex $v$ can be computed in linear time $\Ocal(m+n)$.

Let $T=(V,E)$ be a tree and $\tau$ be a generalized threshold function in $T$. Let $B_0$ be the set of vertices $v$ of $G$ with $\tau(v)>d(v)$.
%\ig{IMPORTANT: in \cref{sec:FPT-Alg}, I have used the notation $V_{\sf f}$ to denote something similar, buy slightly different: a set of \emph{forced} vertices that must belong to the target set, but this vertices have $\tau(v) \leq d(v)$, because in \cref{sec:FPT-Alg} I only consider threshold functions. In fact, the \FPT algorithms also work easily with any function $\tau$, but is it worth to say it?}.
We now explain how to compute $t_{\tau}(T)$ in $O(n^2)$-time.
%using the results of \cref{sec:PolyTrees}.
Start by computing $H(B_0)$ and compute the time $t_{\tau}(v,B_0)$ for every vertex $v$ of $T$. For every vertex $v$ of $H(B_0)$, set $t_{\tau}(v)=t_{\tau}(v,B_0)$.
%For every vertex $v$ of $H(B_0)$ with a neighbor $w\not\in H(B_0)$, set $t_{\tau}(v,w)=t_{\tau}(v,B_0)$. With this, \c{applying \cref{teo1} and \cref{cor1}} \ig{as I mentioned in \cref{sec:PolyTrees}, we also need \cref{lem:recursion}, and a formal result explaining that algorithm}, we can compute $t_{\tau}(w)$ for every vertex $w\in V\setminus H(B_0)$ and compute $t_{\tau}(G)$ in \c{polynomial} \igr{delete} time $\Ocal(n^3)$. From this, we have the following theorem.

%\begin{theorem}\label{thm:poly-trees-general}
%For every tree $G$ and any \c{threshold function} \ig{according to what I proposed, we should not call it ``threshold function''. We could call it a ``generalized threshold function''} \edicao{I AGREE.}{} $\tau:V(G)\to\NN$, \c{the TSS-maxtime} \ig{remove this} $t_{\tau}(G)$ can be computed in time $\Ocal(n^3)$.
%\end{theorem}


%In the following, we present an alternative and \c{more intuitive algorithm} \ig{what follows is really more intuitive...?}. As before, start by computing $H(B_0)$ and compute the time $t_{\tau}(v,B_0)$ for every vertex $v$ of $G$. For every vertex $v$ of $H(B_0)$, \c{we prove that $t_{\tau}(v)=t_{\tau}(v,B_0)$} \ig{but before \cref{thm:poly-trees-general} you have already said this, without a proof}.

For every vertex $v\not\in H(B_0)$ with a neighbor in $H(B_0)$, set the \emph{beginning time}  $b(v)$ of $v$ as $b(v)=\max\{t_{\tau}(w) : w\in N(w)\cap H(B_0)\}$. For the other vertices $v\not\in H(B_0)$, set $b(v)=0$.

Notice that, for every vertex $v\not\in H(B_0)$, $\tau(v)\leq d(v)$.
We say that a vertex $v\in V\setminus H(B_0)$ is \emph{saturated} if $\tau(v)=d(v)$; otherwise, it is \emph{non-saturated}.
Therefore, in the tree $G$, we have three types of vertices: vertices of $H(B_0)$, saturated vertices, and non-saturated vertices.

Clearly a saturated vertex $v$ is activated if and only if it is in the target set or all its neighbors are activated. In other words, a saturated vertex outside the target set cannot help to activate other vertices.

A \emph{non-saturated path} in the tree $G$ is a path such that all its vertices are non-saturated. In the following, we prove that, for every non-saturated vertex $v\in V\setminus H(B_0)$, the maximum time $t_{\tau}(v)$ is equal to the maximum value, among all non-saturated paths $P$ finishing at $v$, of $b(u)+|P|$, where $|P|$ is the number of vertices in the path $P$ and $u$ is the endpoint of $P$ distinct from $v$.
Moreover, for every saturated vertex $w\in V\setminus H(B_0)$, we prove that $t_{\tau}(w)=1+\max\{t_{\tau}(v)\}$ among all non-saturated neighbors $v$ of $w$, if there is one; otherwise $t_{\tau}(w)=1$.


\input{Fig9}

\input{Fig10}


\cref{fig:Fig9} and \cref{fig:Fig10} show an example for the same tree $T$. In both figures, the black vertices are the vertices of $B_0$ (that is, vertices $v$ with $\tau(v)>d(v)$) and the blue vertices are the vertices in $H(B_0)\setminus B_0$. Let $u$ and $v$ be the vertices with label 9 and 16 in \cref{fig:Fig9}, respectively. Notice that all 8 vertices in the path between $u$ and $v$ (light green in both figures) are non-saturated. The numbers inside the black or blue vertices are the values of $t_{\tau}(w)$ of the vertices in $H(B_0)$ in both figures. In this example, we have that $b(u)=8$ and $b(v)=3$. Moreover, $t_{\tau}(u)=3+8=11$ and $t_{\tau}(v)=8+8=16$.
The maximum times 17 and 12 in \cref{fig:Fig9} and \cref{fig:Fig10} are obtained in saturated vertices. The maximum time $t_{\tau}(T)$ is 17 obtained by the target set of \cref{fig:Fig9}.

\begin{lemma}\label{lem:tau-generalized}
%\ig{I think that this should be a lemma}
Let $T$ be a tree, $\tau$ be a generalized threshold function in $T$ and $v\in V(T)$. Let $B_0$ be the set of vertices $u$ of $T$ with $\tau(u)>d(u)$. If $v\in H(B_0)$, then $t_{\tau}(v)=t_{\tau}(v,B_0)$.
If $v$ is non-saturated, then $t_{\tau}(v)=1+\max\{|P|+b(u) : P\mbox{ is a non-saturated path with an endpoint in $v$, where $u$ is the other endpoint}\}$.
If $v$ is saturated and has a non-saturated neighbor, then $t_{\tau}(v)=1 + \max\{t_{\tau}(u) : \mbox{ $u$ is a non-saturated neighbor of $v$}\}$.
If $v$ is saturated and all its neighbors are saturated, then $t_{\tau}(v)=1$.
%\[
% t_{\tau}(v)=
% \begin{cases}
% t_{\tau}(v,B_0), &\mbox{if $v\in H(B_0)$},\\
% 1\ +\ \max\Big\{|P|+b(u)\ :\ P\mbox{ is a non-saturated path from $u$ to $v$}\Big\}, &\mbox{if $v$ is non-saturated},\\
% 1\ +\ \max\Big\{t_{\tau}(u)\ :\ \mbox{ non-saturated neighbors $u$ of $v$}\Big\}, &\mbox{if $v$ is saturated and has a non-saturated neighbor},\\
% 1, &\mbox{if $v$ is saturated and all neighbors are saturated},\\
%  \end{cases}
%\]
\end{lemma}

\begin{proof}
If $v\in H(B_0)$, then, \c{from \cref{lema1}} \ig{IMPORTANT: I don't understand this. \cref{lema1} deals only with ``proper'' threshold function, and where $v$ is a leaf of $G$. Why can it be applied here? Please justify}, it is possible to obtain a target set $S_0$ which contains $B_0$ and such that $t_{\tau}(v,S_0)=t_{\tau}(v,B_0)$ for every $v\in H(B_0)$ and we are done, since every target set must contain $B_0$.

Now recall \c{Theorem 1} \ig{which is this theorem? If it only applies to ``proper'' threshold functions, why can we use it here?}: $t_{\tau}(v)=1+\max\{t_{\tau}(u,v) : u\in N(v)\}$.
Clearly, if $u$ is saturated, then $t_{\tau}(u,v)=0$, since \b{any neighbor} $v$ \b{of $u$} is necessary to activate $u$ at time greater than 0.
Moreover, if $v$ is saturated and $u$ is non-saturated, then $t_{\tau}(u,v)=t_{\tau}(u)$, since $v$ cannot help to activate $u$.
Therefore, if $v$ is saturated and all its neighbors are saturated, then $t_{\tau}(v)=1$.
Moreover, if $v$ is saturated and has at least one non-saturated neighbor, then $t_{\tau}(v)=1+\max\{t_{\tau}(u) : \mbox{ $u$ is a non-saturated neighbor of $v$}\}$.

Finally, consider a non-saturated vertex $v$. Consider a target set $S_0$ which activates $v$ at time $t$. We want to show that there exists a path $P$ of non-saturated vertices with such that $t=b(u)+|P|$ where $u$ and $v$ are the endpoints of $P$. First notice that there exists a path $P'=(u_0,u_1,u_2,\ldots,u_{t-1},v)$ in the tree $G$ of vertices which are activated by $S_0$ at times $0,1,2,\ldots,t-1,t$, respectively.
Since vertices with $\tau(v)\geq d(v)$ cannot help to activate other vertices in time greater than 1, all vertices in the path $P'$, except $u_0$, are such that $\tau(v)<d(v)$ (\b{that is, they} are non-saturated or belong to $H(B_0)$).
We may assume that there exists $0\leq k<t$ such that $u_1,\ldots,u_k$ are in $H(B_0)$ and $u_{k+1},\ldots,u_{t-1}$ are non-saturated. This is because every vertex of $H(B_0)$ with \b{activation} time $k+1$ was activated by a vertex of $H(B_0)$ with \b{activation} time $k$.
Therefore $b(u_{k+1})\geq t_{\tau}(u_k)=k$. The subpath $P=(u_{k+1},\ldots,u_{t-1},v)$ of $P'$ with non-saturated vertices has size $|P|=t-k$. Then the \b{activation} time of $v$ in the process of the target set $S_0$ is equal to $t=k+(t-k)=b(u)+|P|$, where $u=u_{k+1}$ is the endpoint of $P$ distinct from $v$.

Now consider a path $P$ of non-saturated vertices $P=(u_1,\ldots,u_{\ell-1},v)$ with size $|P|=\ell$. We want to show that there exists a target set $S_0$ which activates $v$ at time of $b(u_1)+|P|$.
\c{From \cref{lema1}} \ig{again, we have to explain why we can use this lemma}, we have that there exists a target set which activates $u_1$ at time $b(u_1)+1$. Since $u_1,u_2,\ldots,u_{\ell-1}$ are non-saturated, we have from \cref{lema1} that there exists a target set which activates $u_k$ at time $b(u_1)+k$. Then $v$ can be activated at time $b(u_1)+|P|$, and we are done.
\end{proof}

\ig{IMPORTANT: again, I don't see at all why the following result is a corollary of \cref{lem:tau-generalized}}

\begin{corollary}
Let $G$ be a tree and $\tau:V\to\NN$ \c{be any threshold function} \ig{again, according to what I proposed, we should not call it ``threshold function'', but maybe ``generalized threshold function'', or just ``function''}. Then,
$t_{\tau}(G)=\max\{t_{\tau}(v) : v\in V(G)\}$.
\end{corollary}

\ig{IMPORTANT: again, the PROOF IS MISSING in the above result! We really need to write down a proof that gives an explicit polynomial running time, even if it is not complicated}

\input{Fig11}


